Detecting and measuring human gastric peristalsis using magnetically controlled capsule endoscope

Magnetically controlled capsule endoscope (MCCE) is an emerging tool for the diagnosis of gastric diseases with the advantages of comfort, safety, and no anesthesia. In this paper, we develop algorithms to detect and measure human gastric peristalsis (contraction wave) using video sequences acquired by MCCE. We develop a spatial-temporal deep learning algorithm to detect gastric contraction waves and measure human gastric peristalsis periods. The quality of MCCE video sequences is prone to camera motion. We design a camera motion detector (CMD) to process the MCCE video sequences, mitigating the camera movement during MCCE examination. To the best of our knowledge, we are the first to propose computer vision-based solutions to detect and measure human gastric peristalsis. Our methods have great potential in assisting the diagnosis of gastric diseases by evaluating gastric motility.

==> dummy.tex <==
\subsection{Threshold for camera moving filter}
\begin{figure}[h]
\centering
\includegraphics[width=8cm]{figures/CMFThreshold3.eps}
\caption{(a) The logarithm of mean sequence length over thresholds. After a threshold of 10000, all the frames pass the CMF. (b) The incremental of mean sequence length.}
\label{fig:CMFThreshold}
\end{figure}
Shorter but more stable video sequences are formulated by screening the MCCE dataset using CMF. The consecutive video frames that pass the CMF will be used for training the CNN+LSTM. We applied the CMF to the MCCE dataset and changed the threshold T. We plotted the resulting mean video sequence length against the threshold as shown in Figure \ref{fig:CMFThreshold}. With a higher threshold, the mean sequence length is longer as shown in Figure \ref{fig:CMFThreshold} (a). However, the selected video sequences contain more camera motion if we use higher thresholds. As shown in Figure \ref{fig:CMFThreshold} (b), the mean sequence length increases slower between [200, 800] compared to that of [0, 200]. Thus, a threshold of 200 is adopted for CMF in consideration of the trade-off between the sequence length and camera motion within sequences.

\begin{figure}[h]
\centering
\includegraphics[width=9cm]{figures/RecordingsCopy.eps}
\caption{The prediction (solid lines) and visual inspection (dashed lines) results of each frame in the 4 representative testing recordings: (a)-(d) correspond to 4 representative cases. For each frame in the video sequence, the CNN+LSTM20 model provides a prediction of 'Wave' or 'Nowave'. The visual inspection results are labeled manually for each frame. Two frames last 1s (fps=2s).}
\label{fig:Recordings}
\end{figure}

We apply the CMF and trained CNN+LSTM20 model to the testing set, which is unseen during training and validation. The results of 4 representative cases are shown in Figure \ref{fig:Recordings}. 
%The testing results (blue lines) are in accordance with the visual inspection (red lines) of MCCE video sequences. 
Similar to visual inspection (dashed lines), the testing results (solid lines) are capable of detecting contraction waves in MCCE records. The visual inspection results serve as a reference and they are not the golden standard. We need further investigation to determine whether our ensemble of CNN, LSTM, and CMF outperform visual inspection in detecting contraction waves in the MCCE dataset.

\begin{table}
\centering
\caption{The mean, median, max, and min values of the error between detected and counted period of human contraction waves for the 30 cases.}
\label{table:tab2}
\begin{tabular}{llll} 
\hline
Mean    & Median  & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{Min}  \\ 
\hline
-2.43\% & -6.33\% & +45.38\%                & -22.24\%                 \\ 
\hline
        &         &                         &                         
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Performance of CNN, CNN+LSTM5, CNN+LSTM10, and CNN+LSTM20. The results are averaged based on 5-fold cross-validation. The numbers after LSTM stands for the LSTM length.}
\begin{adjustbox}{width=0.5\textwidth}
\label{table:tab1}
\begin{tabular}{ccccc} 
\hline
\multicolumn{1}{l}{\diagbox{Methods}{Metrics}} & \multicolumn{1}{l}{Accuracy} & Sensitivity & Precision & Specificity  \\ 
\hline
CNN                                            & 81.5\%                       & 70.7\%      & 74.5\%    & 85.1\%       \\
CNN+LSTM5                                      & 85.9\%                       & 75.7\%      & 85.1\%    & 86.6\%       \\
CNN+LSTM10                                     & 87.3\%                       & 77.6\%      & 86.8\%    & 87.9\%       \\
CNN+LSTM20                                     & 87.4\%                       & 78.1\%      & 86.7\%    & 88.1\%       \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}
